PEAR: Primitive Enabled Adaptive Relabeling for Boosting Hierarchical Reinforcement Learning

Hierarchical reinforcement learning (HRL) has the potential to solve complex long horizon tasks using temporal abstraction and increased exploration. However, hierarchical agents are difficult to train due to inherent non-stationarity. We present primitive enabled adaptive relabeling (PEAR), a two-phase approach where we first perform adaptive relabeling on a few expert demonstrations to generate efficient subgoal supervision, and then jointly optimize HRL agents by employing reinforcement learning (RL) and imitation learning (IL). We perform theoretical analysis to bound the sub-optimality of our approach and derive a joint optimization framework using RL and IL. Since PEAR utilizes only a few expert demonstrations and considers minimal limiting assumptions on the task structure, it can be easily integrated with typical off-policy RL algorithms to produce a practical HRL approach. We perform extensive experiments on challenging environments and show that PEAR is able to outperform various hierarchical and non-hierarchical baselines and achieve upto $80\%$ success rates in complex sparse robotic control tasks where other baselines typically fail to show significant progress. We also perform ablations to thoroughly analyse the importance of our various design choices. Finally, we perform real world robotic experiments on complex tasks and demonstrate that PEAR consistently outperforms the baselines.

==> figures/bin_success_visualization_1.tex <==
\begin{figure*}[ht]
\vspace{5pt}
\centering
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_1.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_2.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_3.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_4.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_5.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_6.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing bin task}
\label{fig:bin_viz_success_1_ablation}
\end{figure*}



==> figures/bin_success_visualization_2.tex <==
\begin{figure*}[ht]
\vspace{5pt}
\centering
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_1_viz_1.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_1_viz_2.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_1_viz_3.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_1_viz_4.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_1_viz_5.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_1_viz_6.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing bin task}
\label{fig:bin_viz_success_1_ablation}
\end{figure*}



==> figures/hollow_failure_visualization_1.tex <==
\begin{figure*}[ht]
\vspace{5pt}
\centering
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_3_viz_1.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_3_viz_2.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_3_viz_3.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_3_viz_4.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_3_viz_5.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_3_viz_6.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Failed visualization}: The visualization is a falied attempt at performing hollow task}
\label{fig:hollow_viz_success_1_ablation}
\end{figure*}



==> figures/hollow_success_visualization_1.tex <==
\begin{figure*}[ht]
\vspace{5pt}
\centering
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_0_viz_1.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_0_viz_2.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_0_viz_3.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_0_viz_4.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_0_viz_5.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/hollow_seed_0_viz_6.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing hollow task}
\label{fig:hollow_viz_success_1_ablation}
\end{figure*}



==> figures_tex/algo.tex <==
\label{sec:algorithm}

\begin{minipage}{0.46\textwidth}
\begin{algorithm}[tb]
\caption{Adaptive relabeling}
\label{alg:algo_pear}
%  \hspace*{\algorithmicindent} \textbf{Input:} 
%  $env \:E$, Expert Demonstrations $\mathcal{D}$ , \\
%  \hspace*{\algorithmicindent}
%  \hspace*{\algorithmicindent}\hspace*{\algorithmicindent}Lower level policy $\pi_{l}$ , Upper level policy $\pi_{u}$\\  
%  \hspace*{\algorithmicindent} \textbf{Output:} Upper level expert demonstrations
\begin{algorithmic}
% \Procedure{Careful Parsing}{}
    \STATE Initialize $D_g = \{\}$
    \FOR{each trajectory $e=(s^e_0, s^e_1, \ldots, s^e_{T-1})$ in $\mathcal{D}$}
        \STATE initial state $\leftarrow s^e_0$
        \STATE final goal $\leftarrow g $ %s^e_{T-1}
        \STATE Initialize list of subgoals $D^e_g = \{\}$
        \FOR{i = $1$ \textbf{to} $T-1$}
            \STATE Compute $Q_{\pi^{L}}(s,g=s^e_i,a_i)$
            \IF{$Q_{\pi^{L}}(s,g=s^e_i,a_i) < Q_{thresh}$}
                \STATE $w = i-1$
                \STATE break
            \ENDIF
        \ENDFOR
        \FOR{t = $1$ \textbf{to} $T-1$}
            \FOR{j = $1$ \textbf{to} $w$}
                \STATE Add $s_t,s_{t+j},s_{t+w}$ to $D^e_g$
            \ENDFOR
        \ENDFOR
        \STATE $D_g \leftarrow D_g \cup D^e_g$
    \ENDFOR
\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[tb]
\caption{PEAR}\label{alg:algo_optimization}
% \centering
\begin{algorithmic}
% \Procedure{Careful Parsing}{}
    \STATE Initialize subgoal transition dataset $D_g = \{\}$ 
    \FOR{$i = 1 \ldots N $}
        \IF{$i \% u==0$}
            \STATE Clear $D_g$
            \STATE Populate $D_g$ by relabeling $D$ using PEAR
        \ENDIF
        \STATE Collect off policy experience using $\pi^{H}$ and $\pi^{L}$
        \STATE Update lower primitive via Soft Actor Critic (SAC) and IRL using $D$ (Eq \ref{eqn:joint_update_lower})
        \STATE Sample transitions from $D_g$
        \STATE Update higher policy via SAC and IL using $D_g$ (Eq \ref{eqn:joint_update_upper})
    \ENDFOR
\end{algorithmic}
\end{algorithm}
\end{minipage}

==> figures_tex/bin_success_visualization_1.tex <==
\begin{figure}[ht]
\vspace{5pt}
\centering
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_1.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_2.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_3.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_4.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_5.pdf}}
\fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_6.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing bin task}
\label{fig:bin_viz_success_1_ablation}
\end{figure}



==> figures_tex/dist_ablation.tex <==
\begin{figure}[ht]
% \vspace{5pt}
\centering
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/maze_d_thresh.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/pick_d_thresh.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/bin_d_thresh.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/hollow_d_thresh.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/rope_d_thresh.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/kitchen_d_thresh.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{The success rate plots show the performance of CRISP for various values of $D_{thresh}$ parameter versus number of training timesteps in Column 1 (Maze navigation), Column 2 (Pick and place), Column 3 (Rope manipulation), and Column 4 (Franka kitchen)}
\label{fig:dist_ablation}
\end{figure}



==> figures_tex/dobot_real.tex <==
\begin{figure}[t]
\vspace{1pt}
\centering
\includegraphics[height=2cm,width=1.6cm]{figures/pick_start.pdf}
\includegraphics[height=2cm,width=1.6cm]{figures/bin_start.pdf}
\includegraphics[height=2cm,width=1.6cm]{figures/hollow_start.pdf}
\includegraphics[height=2cm,width=1.6cm]{figures/rope_start.pdf}
\\
\includegraphics[height=2cm,width=1.6cm]{figures/pick_final.pdf}
\includegraphics[height=2cm,width=1.6cm]{figures/bin_final.pdf}
\includegraphics[height=2cm,width=1.6cm]{figures/hollow_final.pdf}
\includegraphics[height=2cm,width=1.6cm]{figures/rope_final.pdf}
\caption{Real world experiments in pick and place (Col 1), bin (Col 2). hollow (Col 3) and rope (Col 4) environments. Row 1 denotes the start and Row 2 denotes final goal configuration.}
\label{fig:dobot_real}
\end{figure}

==> figures_tex/env_collage.tex <==
\begin{figure}[t]
\vspace{5pt}
\centering
\includegraphics[height=5cm,width=5cm]{figures/env_collage.pdf}
\caption{PEAR Overview: While training, both upper policy($\pi^{H}$) and lower primitive($\pi^{L}$) are trained using RL and IL(imitation learning). After every u timesteps, $D_{g}$ is re-populated using PIP.}
% \label{fig:env_collage}
\end{figure}

==> figures_tex/feasible_ablation.tex <==
\begin{figure}[t]
% \begin{minipage}{0.59\textwidth}
\centering
\captionsetup{font=footnotesize,labelfont=scriptsize,textfont=scriptsize}
\subfloat[][Maze]{\includegraphics[scale=0.16]{figures/fig_pear_subgoal_maze.png}}
\subfloat[][Pick and place]{\includegraphics[scale=0.16]{figures/fig_pear_subgoal_pick.png}}
\subfloat[][Bin]{\includegraphics[scale=0.16]{figures/fig_pear_subgoal_bin.png}}
\subfloat[][Hollow]{\includegraphics[scale=0.16]{figures/fig_pear_subgoal_hollow.png}}
\subfloat[][Rope]{\includegraphics[scale=0.16]{figures/fig_pear_subgoal_rope.png}}
\subfloat[][Kitchen]{\includegraphics[scale=0.16]{figures/fig_pear_subgoal_kitchen.png}}
\\
{\includegraphics[scale=0.65]{figures/legend_non_stat_pear.pdf}}
\caption{\textbf{Feasible subgoal generation metric comparison} This figure compares the average distance metric between the subgoals predicted by the higher level policy and the subgoals achieved by the lower level policy after the training is completed. As seen in figure, PEAR consistently produces feasible subgoals which are achievable by the lower level primitive.}
\label{fig:feasible_ablation}
\end{figure}

==> figures_tex/hollow_failure_visualization_1.tex <==
\begin{figure}[H]
\vspace{5pt}
\centering
\captionsetup{font=footnotesize,labelfont=scriptsize,textfont=scriptsize}
\includegraphics[height=1.8cm,width=2.1cm]{figures/hollow_seed_3_viz_1.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/hollow_seed_3_viz_2.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/hollow_seed_3_viz_3.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/hollow_seed_3_viz_4.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/hollow_seed_3_viz_5.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/hollow_seed_3_viz_6.pdf}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Failed visualization}: The visualization is a falied attempt at performing hollow task}
\label{fig:hollow_viz_failure_1_ablation}
\end{figure}



==> figures_tex/kitchen_failure_visualization_1.tex <==
\begin{figure}[h]
\vspace{5pt}
\centering
\captionsetup{font=footnotesize,labelfont=scriptsize,textfont=scriptsize}
\includegraphics[height=1.8cm,width=2.1cm]{figures/kitchen_seed_0_viz_1.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/kitchen_seed_0_viz_2.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/kitchen_seed_0_viz_3.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/kitchen_seed_0_viz_4.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/kitchen_seed_0_viz_5.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/kitchen_seed_0_viz_6.pdf}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Failed visualization}: The visualization is a failed attempt at performing kitchen navigation task}
\label{fig:kitchen_viz_failure_1_ablation}
\end{figure}



==> figures_tex/kitchen_success_visualization_1.tex <==
\begin{figure}[ht]
\vspace{5pt}
\centering
\fbox{\includegraphics[scale=0.07]{figures/kitchen_seed_2_viz_1.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/kitchen_seed_2_viz_2.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/kitchen_seed_2_viz_3.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/kitchen_seed_2_viz_4.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/kitchen_seed_2_viz_5.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/kitchen_seed_2_viz_6.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing kitchen navigation task}
\label{fig:kitchen_viz_success_1_ablation}
\end{figure}



==> figures_tex/margin_ablation.tex <==
\begin{figure}[h]
% \vspace{5pt}
\centering
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/fetchMaze_margin_ablation.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/fetchPick_margin_ablation.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/fetchPickBin_margin_ablation.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/fetchPickHollow_margin.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/rope_margin_ablation.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/kitchen_2_margin.pdf}}
\caption{Column 1 (Maze navigation), Column 2 (Pick and place), Column 3 (Bin), Column 4 (Hollow), Column 5 (Rope manipulation), and Column 6 (Franka kitchen) show success rate performance comparison between PEAR-IRL and PEAR-IRL-Margin ablation. }
\label{fig:margin_ablation}
\end{figure}



==> figures_tex/maze_failure_visualization_1.tex <==
\begin{figure}[ht]
\vspace{5pt}
\centering
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_1_viz_1.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_1_viz_2.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_1_viz_3.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_1_viz_4.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_1_viz_5.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_1_viz_6.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Failed visualization}: The visualization is a failed attempt at performing maze navigation task}
\label{fig:maze_viz_failure_1_ablation}
\end{figure}



==> figures_tex/maze_failure_visualization_2.tex <==
\begin{figure}[h]
\vspace{5pt}
\centering
\captionsetup{font=footnotesize,labelfont=scriptsize,textfont=scriptsize}
\includegraphics[height=1.8cm,width=2.1cm]{figures/maze_seed_6_viz_1.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/maze_seed_6_viz_2.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/maze_seed_6_viz_3.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/maze_seed_6_viz_4.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/maze_seed_6_viz_5.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/maze_seed_6_viz_6.pdf}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Failed visualization}: The visualization is a failed attempt at performing maze navigation task}
\label{fig:maze_viz_failure_2_ablation}
\end{figure}



==> figures_tex/maze_success_visualization_1.tex <==
\begin{figure}[ht]
\vspace{5pt}
\centering
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_0_viz_1.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_0_viz_2.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_0_viz_3.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_0_viz_4.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_0_viz_5.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/maze_seed_0_viz_6.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing maze navigation task}
\label{fig:maze_viz_success_1_ablation}
\end{figure}



==> figures_tex/p_ablation.tex <==
\begin{figure}[ht]
% \vspace{5pt}
\centering
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/maze_populate_num.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/pick_populate_num.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/bin_populate_num.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/hollow_populate_num.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/rope_populate_num.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/kitchen_populate_num.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{In Column 1 (Maze navigation), Column 2 (Pick and place), Column 3 (Rope manipulation), and Column 4 (Franka kitchen) show success rate performance plots of CRISP for different values of hyperparameter $p$, plotted against number of training timesteps.}
\label{fig:p_ablation}
\end{figure}



==> figures_tex/pear_explanation.tex <==
\begin{figure}[t]
\vspace{5pt}
\centering
\includegraphics[height=6cm,width=8cm]{figures/pear_explanation.pdf}
\caption{PEAR Overview: While training, both upper policy($\pi^{H}$) and lower primitive($\pi^{L}$) are trained using RL and IL(imitation learning). After every u timesteps, $D_{g}$ is re-populated using PIP.}
% \label{fig:pear_explanation}
\end{figure}

==> figures_tex/pick_success_visualization_1.tex <==
\begin{figure}[ht]
\vspace{5pt}
\centering
\fbox{\includegraphics[scale=0.08]{figures/pick_seed_2_viz_1.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/pick_seed_2_viz_2.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/pick_seed_2_viz_3.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/pick_seed_2_viz_4.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/pick_seed_2_viz_5.pdf}}
\fbox{\includegraphics[scale=0.08]{figures/pick_seed_2_viz_6.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing pick navigation task}
\label{fig:pick_viz_success_1_ablation}
\end{figure}



==> figures_tex/real_experiments.tex <==
% \begin{figure}[ht]
% \vspace{5pt}
% \centering
% \fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_1.pdf}}
% \fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_2.pdf}}
% \fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_3.pdf}}
% \fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_4.pdf}}
% \fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_5.pdf}}
% \fbox{\includegraphics[scale=0.065]{figures/bin_seed_0_viz_6.pdf}}
% % \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% % \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
% \caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing bin task}
% \label{fig:bin_viz_success_1_ablation}
% \end{figure}



\begin{figure}[ht]
% \begin{minipage}{0.37\textwidth}
\centering
\captionsetup{font=footnotesize,labelfont=scriptsize,textfont=scriptsize}
% \captionsetup[subfloat]{labelfont=scriptsize,textfont=scriptsize}
\includegraphics[scale=0.1]{figures/pick_start.pdf}
\hspace{0.005cm}
\includegraphics[scale=0.1]{figures/bin_start.pdf}
\hspace{0.005cm}
% \includegraphics[scale=0.1]{figures/hollow_start.pdf}
\includegraphics[scale=0.1]{figures/rope_start.pdf}

\subfloat[][Pick and place]{\includegraphics[scale=0.1]{figures/pick_final.pdf}}
\hspace{0.1cm}
\subfloat[][Bin]{\includegraphics[scale=0.1]{figures/bin_final.pdf}}
% \includegraphics[scale=0.1]{figures/hollow_final.pdf}
\hspace{0.1cm}
\subfloat[][Rope]{\includegraphics[scale=0.1]{figures/rope_final.pdf}}
\caption{\textbf{Real world experiments} in pick and place, bin and rope manipulation environments. Row 1 depicts initial and Row 2 depicts goal configuration.}
\label{fig:dobot_real}
% \end{minipage}
\end{figure}

==> figures_tex/rope_failure_visualization_1.tex <==
\begin{figure}[ht]
\vspace{5pt}
\centering
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_3_viz_1.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_3_viz_2.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_3_viz_3.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_3_viz_4.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_3_viz_5.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_3_viz_6.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Failed visualization}: The visualization is a failed attempt at performing rope navigation task}
\label{fig:rope_viz_failure_1_ablation}
\end{figure}



==> figures_tex/rope_failure_visualization_2.tex <==
\begin{figure}[h]
\vspace{5pt}
\centering
\captionsetup{font=footnotesize,labelfont=scriptsize,textfont=scriptsize}
\includegraphics[height=1.8cm,width=2.1cm]{figures/rope_seed_8_viz_1.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/rope_seed_8_viz_2.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/rope_seed_8_viz_3.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/rope_seed_8_viz_4.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/rope_seed_8_viz_5.pdf}
\includegraphics[height=1.8cm,width=2.1cm]{figures/rope_seed_8_viz_6.pdf}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Failed visualization}: The visualization is a failed attempt at performing rope navigation task}
\label{fig:rope_viz_failure_2_ablation}
\end{figure}



==> figures_tex/rope_success_visualization_1.tex <==
\begin{figure}[ht]
\vspace{5pt}
\centering
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_5_viz_1.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_5_viz_2.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_5_viz_3.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_5_viz_4.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_5_viz_5.pdf}}
\fbox{\includegraphics[scale=0.07]{figures/rope_seed_5_viz_6.pdf}}
% \includegraphics[scale=0.3, height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{\textbf{Successful visualization}: The visualization is a successful attempt at performing rope navigation task}
\label{fig:rope_viz_success_1_ablation}
\end{figure}



==> figures_tex/success_rate_comparison.tex <==
\begin{figure}[t]
\vspace{1pt}
\centering
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/maze_success_rate.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/pick_success_rate.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/bin_success_rate.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/hollow_success_rate.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/rope_success_rate.pdf}}
\fbox{\includegraphics[height=1.5cm,width=2cm]{figures/kitchen_success_rate.pdf}}
% \fbox{\includegraphics[height=2cm,width=2cm]{figures/pick_distance.pdf}}
% \fbox{\includegraphics[height=2cm,width=2cm]{figures/rope_distance.pdf}}
% \includegraphics[height=4cm,width=12cm]{figures/train_test_val_collage_final.pdf}
% \includegraphics[scale=0.2]{figures/eight_room_success_rate_comparison.pdf}
\caption{The success rates plots of PEAR-IRL, PEAR-BC and other baselines in maze navigation (Col. 1), pick and place (Col. 2), bin (Col. 3), hollow (Col. 4), rope manipulation (Col. 5), and kitchen environment (Col. 6) vs number of timesteps.}
\label{fig:success_rate_comparison}
\end{figure}


==> figures_tex/tbl_performance.tex <==
\begin{table}[ht!]
\vspace{5pt}
\caption{Success rate comparison}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|P{1.3cm}|P{1.5cm}|P{1.5cm}|P{1.5cm}|P{1.5cm}|}
% \begin{tabular}{|P{2.7cm}|P{1.645cm}|P{1.645cm}|P{1.645cm}|P{1.645cm}|}
% \resizebox{\textwidth}{!}{%
\centering
\adjustbox{max width=0.85\textwidth}{%
\begin{tabular}{@{}c*{6}{c}@{}}
% {|P|P|P|P|P|P|P|}

% {|P{1.7cm}|P{1.645cm}|P{1.645cm}|P{1.645cm}|P{1.645cm}|P{1.645cm}|P{1.645cm}|}
 \hline
 & Maze & Pick Place & Bin & Hollow & Rope & Kitchen  \\ \hline
PEAR-IRL & \textbf{0.84 $\pm$ 0.04} & \textbf{0.92 $\pm$ 0.02} & \textbf{0.79 $\pm$ 0.05} & \textbf{0.78 $\pm$ 0.27} & \textbf{0.33 $\pm$ 0.04} & \textbf{0.89 $\pm$ 0.06}  \\ 
PEAR-BC & 0.67 $\pm$ 0.07 & \textbf{0.48 $\pm$ 0.3} & \textbf{0.38 $\pm$ 0.19} & \textbf{0.33 $\pm$ 0.03} & \textbf{0.32 $\pm$ 0.04} & \textbf{1.0 $\pm$ 0.0}  \\ 
RPL & 0.58 $\pm$ 0.09 & 0.28 $\pm$ 0.17 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.13 $\pm$ 0.07 & 0.08 $\pm$ 0.1  \\ 
HAC & 0.6 $\pm$ 0.23 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 0.1 $\pm$ 0.0 & 0.02 $\pm$ 0.01 & 0.0 $\pm$ 0.0  \\ 
RAPS & \textbf{0.81 $\pm$ 0.06} & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & - & 0.0 $\pm$ 0.0  \\ 
HIER-NEG & 0.01 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0 & 0.01 $\pm$ 0.0 & 0.0 $\pm$ 0.0  \\ 
HIER & 0.02 $\pm$ 0.02 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0 & 0.01 $\pm$ 0.0 & 0.0 $\pm$ 0.0  \\ 
DAC & 0.02 $\pm$ 0.02 & 0.21 $\pm$ 0.06  & 0.14 $\pm$ 0.09  & 0.0 $\pm$ 0.0  & 0.03 $\pm$ 0.01 & 0.0 $\pm$ 0.0  \\ 
FLAT & 0.01 $\pm$ 0.01 & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0  & 0.0 $\pm$ 0.0 & 0.03 $\pm$ 0.01 & 0.0 $\pm$ 0.0  \\ 
BC & 0.0 & 0.0 & 0.0 & 0.0 & 0.15 & 0.0 \\ 
% Nearest Neighbour  &  &  &  &  \\
% Interpolation  &  &  &  &  \\ 
\hline


% \textbf{Method} & \textbf{Rope Manipulation}  \\ \hline
% CRISP-IRL                & \textbf{0.29 $\pm$ 0.04}   \\ \hline
% CRISP-BC                    & \textbf{0.32} $\pm$ \textbf{0.056}       \\ \hline
% RPL                      & 0.18 $\pm$ 0.12                \\ \hline
% Hier                       & 0.1 $\pm$ 0.07               \\ \hline

\end{tabular}}
\label{tbl:success_rate_performance}
\end{table}

% \begin{table}[!htbp]
% \adjustbox{max width=\textwidth}{%
% \centering
% \begin{tabular}{@{}l*{6}{c}@{}}
% % {|P|P|P|P|P|P|P|}
%  & Maze & Pick Place & Bin & Hollow & Rope & Kitchen  \\ \hline
% PEAR-IRL & \textbf{0.84 $\pm$ 0.04} & \textbf{0.92 $\pm$ 0.02} & \textbf{0.79 $\pm$ 0.05} 
% \end{tabular}}
% \caption{Proposta de preço para item 1}
% \label{PropostaItem1}
% \end{table}

==> figures_tex/tbl_real_experiments.tex <==
\begin{table}[h]
\vspace{5pt}
\centering
\caption{Success rate comparison}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|P{1.3cm}|P{1.5cm}|P{1.5cm}|P{1.5cm}|P{1.5cm}|}
% \begin{tabular}{|P{2.7cm}|P{2.0cm}|P{2.0cm}|P{2.0cm}|P{2.0cm}|}
\begin{tabular}{|P{2.5cm}|P{2.0cm}|}
 \hline
 & Successes \\ \hline
PEAR-IRL(ours) & 3$/$10  \\ 
PEAR-BC(ours) & 3$/$10 \\ 
RPL & 0$/$10  \\ 
\hline


\end{tabular}
\label{tbl:real_experiments}
\end{table}
